Computing and Exploiting Document Structure to Improve Unsupervised Extractive Summarization of Legal Case Decisions

Though many algorithms can be used to automatically summarize legal case decisions, most fail to incorporate domain knowledge about how important sentences in a legal decision relate to a representation of its document structure. For example, analysis of a legal case summarization dataset demonstrates that sentences serving different types of argumentative roles in the decision appear in different sections of the document. In this work, we propose an unsupervised graph-based ranking model that uses a reweighting algorithm to exploit properties of the document structure of legal case decisions. We also explore the impact of using different methods to compute the document structure. Results on the Canadian Legal Case Law dataset show that our proposed method outperforms several strong baselines.

==> EMNLP -- Legal Summarization-3/Sections/Conclusion.tex <==
\section{Conclusion}
We presented an unsupervised graph-based model
for the summarization of long legal case decisions. Our
proposed approach incorporated diverse views of the document structure of legal cases and utilized a reweighting scheme to better select argumentative sentences. Our exploration of document structure demonstrates how using different types of document structure impacts summarization performance. Moreover, a document structure inspired reweighting scheme yields  performance gain on the CanLII case dataset.

\section*{Ethical Considerations}
The utilization of the generated summary results of legal documents remains important. Current extractive methods avoid the problem of generating hallucinated information \cite{kryscinski-etal-2020-evaluating,maynez-etal-2020-faithfulness}, which has been observed in abstractive methods that use large-scale pre-trained language models. The extracted sentences, however, may not capture the important contents of the legal documents.
Meanwhile, CanLII has taken measures to limit the disclosure of defendants' identities (such as blocking search indexing). Thus, using the dataset may need to be taken good care of and avoid impacting those efforts. 

\section*{Acknowledgement}
We thank the Pitt AI Fairness and Law group,
the Pitt PETAL group, and the
anonymous reviewers for their valuable feedback.
This research is supported by
the National Science Foundation under Grant IIS-2040490 and a gift from Amazon.

\section*{Limitations}
%We acknowledge several limitations of this work.
The dataset we used has a relatively small scale (1K) 
test set. Meanwhile, the automatic evaluation metrics may fall short compared to human evaluations, %in identifying the synonyms of legal terminologies, 
thus unfaithfully representing the final quality of generated summaries. Although lightweight, there is still a large performance gap between our unsupervised method and both the extractive oracles as well as abstractive models (Appendix \ref{sec:appendix_abstractive}), especially given the small-scale training data. There are more graph-based methods to aggregate information from the built graphs and we would like to explore and include more graph-based methods but selected the most relevant one in this work.
Moreover, our proposed reweighting paradigm heavily relied on observations about the structure of legal cases. Many other legal document types, such as bills and statutes, have inherently distinct structures. Our results also show the importance of finding the correct  structure and  weights, which can vary depending on the corpus. This will require more advanced methods to find the correct structure and weights for a dataset.



==> EMNLP -- Legal Summarization-3/Sections/Dataset.tex <==
\section{Case Decision Summarization Dataset}\label{sec:dataset}
Recent work has introduced a number of legal document summarization or salient information identification tasks with associated datasets, e.g., for bill %or case 
summarization %\cite{kornilova-eidelman-2019-billsum, malik2021semantic} 
\cite{kornilova-eidelman-2019-billsum}
and for case sentence argumentive classification \cite{xu-2021-position-case} and rhetorical role prediction
\cite{malik2021semantic}.
%However, unlike the news and scientific articles, only limited amount of annotated data point are available and the size is of orders of magnitude smaller. 
\begin{table}[t!]
% \small
% \scriptsize 
    \centering
    % \setlength\tabcolsep{2.1pt}
    \renewcommand{\arraystretch}{1}%Tighter
    \begin{tabular}{l|c}
    
    %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
   \toprule
 %  &  CanLII  \\
 %\midrule
    Case length (avg. \# words) & 3,971\\
    Summary length  (avg. \# words) & 266\\
    Training set  (\# case/summary pairs) & 27,241 \\
    
    Testing set  (\# case/summary pairs) & 1,049\\
    
%      Name & Size & Doc. len & Summ. len. \\
%     \midrule
%     BillSum & 22,218 & 1,592 &  197 \\
%   CanLII & 28,290 & 3,971   &  266 \\
%   \midrule
%     XSum & 226k &  431 & 23 \\
%     CNN/DM &  311k & 766 & 53 \\
%     \midrule
%     PubMed  & 133k  &  3,016 & 203 \\
%     arXiv &  215k & 4,938 & 220 \\
    \bottomrule
    \end{tabular}
    \caption{Dataset statistics of CanLII.}
    \label{tab:data_stats}
\end{table}
\begin{figure}[t!]
\centering
 \includegraphics[width=.9\linewidth]{Figs/IRC_distribution.png}

  \caption{Fraction of sentences annotated as argumentative (using the IRC scheme) in the case documents versus in the summaries of the CanLII test set. Though only a small fraction of sentences in the original document are annotated as IRCs, IRCs are a large fraction of the human-written summaries.}
  \label{fig: disbribution}
\end{figure} 
Similarly to \citet{xu-2021-position-case}, we use the {\bf CanLII} (Canadian Legal Information Institute) dataset of legal case decisions and summaries\footnote{The data was obtained through an agreement with the Canadian Legal Information Institute (CanLII) (\url{https://www.canlii.org/en/}).}. 
%Persons interested in accessing the data should contact CanLII directly.}.   %Kevin suggested this wording
%\footnote{The data can be obtained through a license agreement with the Canadian Legal Information Institute (\url{https://www.canlii.org/en/}).}%\footnote{We provide examples from this dataset in Appendix \ref{appendix:output}.} 
  Full corpus statistics are provided in Table \ref{tab:data_stats}, while an example case/summary pair from the test set is provided in Figure \ref{fig:IRC_example} in Appendix \ref{appendix:1}.
%ref{appendix:output}.
%\\
    % (1) \textbf{BillSum}\footnote{\url{https://github.com/FiscalNote/BillSum}} \cite{kornilova-eidelman-2019-billsum}, which contains 22,218 US Congressional Bills with human-written references and has been split into 18,949 train bills and 3,269 test bills. \\
%\textbf{CanLII}  
%of the non-profit Canadian Legal Information Institute\footnote{\url{https://www.canlii.org/en/}}. 

\citet{xu-2021-position-case} only used a small portion of this dataset for their work in argumentative classification. Conjecturing that explicitly identifying the decision's argumentative components would be crucial in case summarization,  they annotated 1,049  case and human-written summary pairs curated from the full dataset.
%CanLII Connects website\footnote{\url{https://canliiconnects.org/en}}. %\citet{xu-2021-position-case}
In particular, they recruited legal experts to annotate the document on the sentence level, adopting an \textbf{IRC scheme} (see Figure \ref{fig:IRC_example} in Appendix \ref{appendix:1}) which classifies individual sentences into one of  four categories: \textbf{Issue} (legal question  addressed in the case), \textbf{Conclusion} (court’s decisions for the corresponding issue), \textbf{Reason} (text snippets explaining why the court made such conclusion) and \textbf{Non\_IRC} (none of the above). The distributions of the IRC labels in  the cases and summaries are shown in Figure \ref{fig: disbribution} and illustrate that argumentative sentences do indeed play an important role in human summaries. We utilized the unannotated 27,241  pairs to train a  supervised model baseline and the 1049 annotated pairs as our test set.  While none of our summarization methods  use the IRC annotations, they are used during testing as the basis of a domain-specific evaluation metric.

%For comparison, the statistics of the commonly used mews and scientific domain summaries are also included \cite{nallapati-etal-2016-abstractive, narayan-etal-2018-dont, cohan-etal-2018-discourse}.  



% \begin{table}[t!]
% % \small
% % \scriptsize 
%     \centering
%     % \setlength\tabcolsep{2.1pt}
%     \renewcommand{\arraystretch}{1}%Tighter
%     \begin{tabular}{c|c| cc}
    
%     %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
%     \toprule
%      Name & Size & Doc. len & Summ. len. \\
%     \midrule
%     BillSum & 22,218 & 1,592 &  197 \\
%   CanLII & 28,290 & 3,971   &  266 \\
% %   \midrule
% %     XSum & 226k &  431 & 23 \\
% %     CNN/DM &  311k & 766 & 53 \\
% %     \midrule
% %     PubMed  & 133k  &  3,016 & 203 \\
% %     arXiv &  215k & 4,938 & 220 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Dataset statistics on legal documents (BillSum and CanLII), news articles (CNN/Daily Mail and XSum
% ) and long scientific documents (PubMed and arXiv).}
%     \label{tab:data_stats}
% \end{table}


==> EMNLP -- Legal Summarization-3/Sections/Introduction.tex <==
\section{Introduction}
Single document summarization aims at rephrasing a long text into a shorter version while preserving the important information \cite{INR-015}. While recent years have witnessed a blooming of abstractive summarization models that can generate fluent and coherent new wordings %and obtain high automatic evaluation scores %compared to human written summaries
\cite{rush-etal-2015-neural, zhang2020pegasus, lewis-etal-2020-bart},  abstractive %struggle to preserve the factual inconsistency.Such models can 
 summaries often contain hallucinated facts %which are not supported by the original source text 
 \cite{kryscinski-etal-2019-neural}. In contrast, extractive summarization models directly select sentences/phrases from the source document to form a summary. In certain domains such as the law or science \cite{bhattacharya2019comparativestudy,dong-etal-2021-discourse}, using  exact wordings may be needed. 

In this work, we focus on {\it extractive summarization of legal case decisions}. Different from texts in the news domain, case texts tend to be longer  (e.g., in Canadian legal case decisions \cite{xu-2021-position-case} there are on average  3.9k words, while standard news articles \cite{nallapati-etal-2016-abstractive} range from 400 - 800 words) and also have more complicated document structures (e.g., legal cases are likely to be split into sections while news articles are not). %It is also infeasible to expect that 
In contrast to scientific domains, which also have long and structured texts, large %scale %and high-quality
training sets of case decisions and reference summaries are generally not freely  available given the restrictions of the legal field.  %For example, 
A currently used case %decision %"appellate court decision" 
dataset has less than 30k training examples \cite{xu-2021-position-case}, which is ten times less than scientific datasets such as arXiv and PubMed \cite{cohan-etal-2018-discourse}. Thus, for the legal domain, it is not surprising that {\it unsupervised} extractive summarization methods are of %particular 
interest. %for the legal domain, %come to be the subject of usage. 
%Traditional unsupervised extractive models use 
%such as graph-based algorithms than  rank sentences based on an importance score. For the legal documents,  
Unfortunately, when researchers \cite{sarvanan-2006-graphical, bhattacharya2019comparativestudy} have attempted to directly apply standard unsupervised %extractive summarization 
models %(e.g., graph-based algorithms that  rank sentences based on an importance score) 
to legal data, they have obtained  mediocre results.  

However, most such attempts have failed to utilize the \textit{document structure
of legal texts}.
%For example, 
In case law, %documents, 
important sentences about the issues versus the decisions of the court occur in different places in the document structure.
In contrast,  summarization algorithms typically flatten any structure during initial processing (i.e., they concatenate sentences from different sections/paragraphs of a document to form a sentence list),
%More recent domain-agnostic 
%Algorithms such as PACSUM \cite{zheng-lapata-2019-sentence} instead 
or select sentences using structural biases from other domains (e.g., the importance of leading sentences in news \cite{zheng-lapata-2019-sentence}).
%which is incapable of dealing with the complicated scenario of legal documents (argumentative sentences such as the issue and decision presented by the court are distributed uniformly in the article). 
As shown in Figure \ref{fig:output_figure}, while %the 
LexRank %algorithm
\begin{figure}[t]
\centering
 \includegraphics[width=1.02\linewidth]{Figs/doc_fig.001.jpeg}

  \caption{An example %CanLII 
  case law document-summary pair (ID: 3\_2000canlii19612) and different summarization system outputs, where sentences are annotated with \textit{argumentative}  \textcolor{red}{Issue}, \textcolor{reasonblue}{Reason}, and \textcolor{conclusiongreen}{Conclusion} labels. Our %proposed
  method better extracts  argumentative sentences from the source document by exploiting its structure.} %For example, one simple way to split the example document into text segments is to use %sentences with the bold and capitalized section names (e.g., BASIS OF CLAIM separating the header information from the main text) as segment boundaries. }
  \label{fig:output_figure}
\end{figure}
correctly extracts the legal issue from the beginning of the source text, it incorrectly extracts several redundant sentences (i.e., %neighboring sentences starts with 
\textit{[20], [21]} and \textit{[22]} %are all selected, which in fact 
which talk about similar content) as well as ignores a large part of the article (e.g., no sentences are extracted from the last section of the original case: \textit{RECAPITULATION OF CALCULATION OF DAMAGES}). In contrast, the human  summary focuses on sentences related to the argument of the legal decision (e.g., what are the issues, reasoning and conclusions of this court case?), which tend to be spread across the document structure. % (which in turn be  computed using different segmentation algorithms such as HMMs or even bolding and capitalization heuristics). 
%More recent domain-agnostic algorithms such as PACSUM \cite{zheng-lapata-2019-sentence}, instead utilized the leading bias of selection of the news domain data, which is incapable of dealing with the complicated scenario of legal documents (argumentative sentences such as the issue and decision presented by the court are distributed uniformly in the article). 

%The only work that starts utilizing the document structure, 
Recently, the  HipoRank model was proposed to  exploit discourse structure patterns during unsupervised extractive summarization \cite{dong-etal-2021-discourse}.  However, the model was designed for  long scientific articles, and the experiments were based on data where the articles were already split into document sections.   %segemented which has a more explicit organization of contents through section segmentation and looser connection across sections. 
For case decisions,  document structures are generally either missing or only implicitly conveyed by text formatting.  For example, in Figure \ref{fig:output_figure}, document  sections are conveyed by bolding in the source HTML file. %, which are typically ignored in summarization data processing. 
Moreover, algorithms such as PACSUM and HipoRank compute  sentence centrality just once and greedily select the top-k candidates %to %extract sentences. 
as the extractive summary. 
%Our pilot study on one of the legal case summarization dataset \cite{xu-2021-position-case} unveils the drawback of such method, as argumentative sentences in legal cases tend to have a uniform distributions and they have higher semantic similarities. 
Such a greedy {selection algorithm} fails to match the distribution of the argumentative sentences that ultimately appear in human case law summaries. %  (recall Figure \ref{fig:output_figure}). 
%and generates low quality summaries. 


To address these limitations, we investigate the utility of different methods for %computing  document structure that %derived from the source text 
%to 
 automatically % model the %hierarchical 
segmenting the sentences of legal case decisions into the sections of a document structure. We posit that incorporating {\it better views of  document structure} could bring improvements in summarization quality
when discourse-aware methods such as HipoRank are applied to legal case decisions.
%Similar to \cite{dong-etal-2021-discourse}, we built document graph with directionality (location relationship between sentences) and hierarchy (section to sentence) to reflect the rich
%document structure of long legal documents.
We also propose a novel \textit{reweighting algorithm} to improve how HipoRank selects sentences when creating extractive summaries of legal decisions.  The algorithm
%We further propose a novel reweighting algorithm, which 
takes the history of already selected summary sentences into account, and gradually updates the importance score of a sentence.  We posit that reweighting will  decrease the selection of  redundant sentences as well as increase the selection of argumentative sentences from less-represented document segments (e.g.,  in the middle).

We evaluate our proposed method\footnote{Our code is available at \url{https://github.com/cs329yangzhong/DocumentStructureLegalSum}} for summarizing legal decisions using an annotated  Canadian case summarization dataset (CanLII) \cite{xu-2021-position-case}. Based on the belief that \textit{argumentative sentences} will capture the important sentences to summarize in a legal decision \cite{xu-2021-position-case,elaraby-litman-2022-arglegalsumm}, a portion of the CanLLI dataset comes with gold-standard sentence-level labels identifying which sentences are related to the issue/reasoning/conclusion of the court's decision in both source and summary documents. We use these labels to additionally propose a  metric that can better evaluate the quality of the generated summary from a legal expert's perspective. 
Empirical results show that our method
improves performance over previous unsupervised
models \cite{zheng-lapata-2019-sentence, dong-etal-2021-discourse, erkan2004lexrank} in automatic evaluation. 


==> EMNLP -- Legal Summarization-3/Sections/Methods.tex <==
\section{Method and Models}
We propose a reweighting model that employs a %simple 
graph-based ranking algorithm to exploit the %document 
structures encoded in long legal case decisions. %.  
%Our method is inspired by the two-level hierarchy design from long scientific article summarization \cite{dong-etal-2021-discourse} and early summarization work tailored for legal document structures \cite{farzindar-lapalme-2004-legal}.

\subsection{Discourse-Aware Backbone Model}\label{sec:main_paper_hiporank}
The HipoRank (Hierarchical and Positional Ranking) model recently developed by \citet{dong-etal-2021-discourse} constructs a directed graph for document representation using document section and sentence hierarchies.
%\footnote{We include a more detailed introduction of the algorithm in Appendix \ref{sec:hiporank}.}. 
HipoRank computes the centrality score of each sentence as 
\begin{equation}
    c(s_i^{I}) = \mu_1 c_{inter} (s_i^{I}) + c_{intra}(s_i^{I})
\end{equation} where $s_i^{I}$ refers to the $i$-th sentence in $I$-th section. $\mu_1$ is a tunable hyper-paramter, $c_{inter}(s_i^{I})$ computes the sentence's similarity to other section representations and  $c_{intra}(s_i^{I})$ computes the average similarity of the current sentence with all others in the same section. 
%, we refer to the original article. 
HipoRank then selects the top-K ranked sentences as the  summary. More details of the algorithm are provided in Appendix \ref{sec:hiporank}.
Directly applying HipoRank to our data yielded multiple challenges (e.g.,  redundant neighboring sentences %based on computed scores
(recall Figure \ref{fig:output_figure}) as well as too many sentences from the ends of the article were selected).

\subsection{Multiple Views of Document Structure}\label{sec:views}

Before creating a HipoRank %hierarchical 
document graph, 
the document must be split into sections and sentences. %Although HipoRank is agnostic to the %section/sentence 
%splitting methods, 
The scientific %document 
datasets previously used with HipoRank %in the HipoRank study 
were already split \cite{dong-etal-2021-discourse}.   We investigate {\it the summarization impact of using different approaches to automatically compute linear sections of the document structure}.
%in the same section.}.
Figure~\ref{fig:three_view} shows different structures for the same  case.
%\footnote{We reprocessed the original HTML files to obtain the original document structures, which may lead to minor sentence formatting problems comparing to the other two structures that used non HTML data preprocessed by \citet{xu-2021-position-case}.}. % can be found in 
%Appendix \ref{apendix:three_views}.

\textbf{Original Document Structure}
This approach extracts the structure by processing the %raw 
{\it HTML files}. We use a heuristic to mark the section names with an italic and bold format as the %section
boundaries and segment the documents into multiple continuous sections. It is worth noting that 297 of the 1049 test case documents do not come with explicit section splits, thus we treat them as whole text spans\footnote{The Original Structure method processed HTML source files and split sentences using a legal %domain-specific 
sentence splitter (\url{https://github.com/jsavelka/luima_sbd}). The Topic and Thematic views used non-HTML data preprocessed by \citet{xu-2021-position-case}, but used the same sentence splitter.}.
%\footnote{We use the sentence splitter from \url{https://github.com/jsavelka/luima_sbd}, as is used in the original CanLII dataset \cite{xu-2021-position-case}.}.

%\paragraph
\textbf{Topic Segment View} Meanwhile, we also explore using a traditional, {\it domain-independent linear text segmentation} algorithm. We use  C99 \cite{choi-2000-advances} but with advanced sentence representation from SBERT \cite{reimers-gurevych-2019-sentence} to group neighboring sentences into topic blocks. %We represent the sentences with
%recent advanced sentence representations using SBERT \cite{reimers-gurevych-2019-sentence}.

\textbf{Thematic Stage View}
Early studies found that legal documents tend to have well-defined, 
{\it domain-dependent thematic structures} \cite{farzindar-lapalme-2004-legal} or rhetorical roles \cite{saravanan-etal-2008-automatic}. Following work that extracts stage views in conversations (introductions → problem exploration →
problem solving → wrap up) \cite{chen-yang-2020-multi}, we extract thematic stages
through a Hidden Markov Model (HMM). A fixed order of stages is imposed and only consecutive transitions are allowed between neighboring stages.  We again represent the sentences %with recent advanced sentence representations 
using SBERT \cite{reimers-gurevych-2019-sentence} and set the number of stages as 5, including the starting Decision Data, Introduction, Context, Judicial Analysis, and Conclusion, as introduced by \citet{farzindar-lapalme-2004-legal}. 
 
 \begin{figure*}[t!]
\centering
 \includegraphics[width=0.85\linewidth]{Figs/three_views.001.jpeg}
  \caption{Different document structure views of a legal case decision (ID: c\_2003skpc17) from our CANLLI test set. Original case sentences are annotated with \textcolor{red}{Issue}, \textcolor{reasonblue}{Reason}, and \textcolor{conclusiongreen}{Conclusion} labels. On the left side, the \textcolor{green}{green}, \textcolor{yellow}{yellow} and \textcolor{cyan}{blue} boxes refer to thematic stage, topic segmentation and the original document structure, respectively. The boxes mean the corresponding sentences on the right hand side are grouped into the same segments. For instance, for the first blue box, the original article is split by the italicized and bolded section name of ``The Fact''. }
  \label{fig:three_view}
\end{figure*}

\textbf{CanLII Header Removing}\label{sec:header_removing} Preliminary analysis demonstrated that the raw CanLII documents fail to distinguish the less important headers at the beginning  (i.e., the descriptive text before the main  content, for example,  the content above the grey splitting line and BASIS OF CLAIM in Figure \ref{fig:output_figure}). Generated summaries also tend to cover  a large portion of such information. We thus propose a legal case decision preprocessing procedure following certain heuristics\footnote{See Appendix \ref{sec:appendix_heuristics} for details.} to remove those headers, and demonstrate the improved summarization quality (for all views of document structure) in Section \ref{sec:result}. 

%We process the original articles into different sections using these three different document structures (one example in Figure \ref{fig:three_view}), and experiment with the state-of-the-art unsupervised extractive baseline HipoRank \cite{dong-etal-2021-discourse} model.


 
% We illustrate the effects of the three methods of document segmentation in Figure \ref{fig:three_view}. It is worth noting that, comparing to the original document structure split by section names, the topic segmentation will produce more fine-grained subparts. But different strategies to segment the document can have diverse effects. For instance, for the highlighted first blue segments, the \textit{issue} sentence is grouped together with all previous headers. Meanwhile, as shown in the last highlighted yellow span, the \textit{reason} sentence is connected with its neighboring sentences, thus can aid for better contextual representation. 

% TODO: Start with hiporank with different inputs.
% TODO: Section 2 reweighting (ours)
%  Yet, there exists drastic difference between the scientific domain and legal domain.  

\subsection{Reweighting the Centrality Score}\label{sec:dynamic_selection}


%Secondly, the original algorithm computed the sentence centrality score only once and greedily select the top-K ranked sentences as the summary. Our analysis \ref{sec:analysis} demonstrate that such approach fail to select sentences in the middle of context which are less similar to others, but carrying the \textit{reasoning} argument role of the legal case. % To tackle the problem of selecting headers (the meta data of the case, as shown in Figure  and the difficulty of reasoning sentences,
% we thus introduce a novel iterative reweighting framework that dynamically update the weights of the candidate nodes based on already selected sentences ( \S \ref{sec:dynamic_selection}). 

% \subsection{Legal Document Summarization}\label{sec:difference}

% \subsection{Hierarchical Directed Graph for legal document}
% Most existing work (TextRank, LexRank, PacSum) build the graph by only considering the sentence similarity and relative order of sentences in the document, which fails to capture the rich document structure of texts. \citet{dong-etal-2021-discourse} introduces a two-level directed hierarchical model that explicitly models the section structures in the scientific articles.

% Different from the clear organizations of sections in scientific articles, the legal case documents sometimes do not come with well-structured format, we instead utilize the multi-views extracted from \S \ref{sec:views}. Similar to prior work, HipoRank formulated the  summarization generation
% as a node selection problem, where those
% nodes (i.e., sentences) that are semantically similar
% to others are picked in the final summary. They proposed a section-level hierarchy, based on the assumption that sentences belonging to different sections are less similar and instead used a section embedding to model the sentence to other section relationship, thus reducing the cost of computation. Different from the strict restrictions on the cross-section sentence edges, we allow for randomized sentence-to-sentence edges, aiming at avoiding the negative effects of under-representation of section. We additionally introduce the weighted parameters to model the distance between either sentence-section or sentence-sentence edges, as inspired by \cite{liu-sigir-2021-distance}.


%Another drawback of 
The HipoRank document graph %built by HipoRank %is that it 
will not change once built, and the important sentences are greedily selected based on the aggregated centrality scores. %Such a method 
This may introduce redundancies in selecting similar sentences and ignore the contents in the middle of the source case decisions that are more important once the argumentative sentences at the beginning and end are taken into account. We propose a novel reweighting approach that can tackle this problem. A prior attempt \cite{tao2021unsupervised}  on multi-round selection looked at the local similarity between %those 
selected sentences. They iteratively recompute the sentence to sentence similarities between the selected summary sentences and recompute the final sentence centrality scores after each sentence selection. Instead, we are focusing on modeling  the relationship between the selected sentence and the other candidate sentences.  Their method is also not directly applicable to longer text due to the $n^2$ time complexity of computation given large numbers of sentences (on average 205 sentences for CanLII dataset). 
\begin{algorithm}
\caption{Reweighting Algorithm}\label{alg:cap}
\begin{algorithmic}
\Require computed centrality score $c(s_i^{I})$ for all sentence s, $c_{intra}(d)$ for different section d 's embedding, and a threshold \textit{g} for phase transition and maximum summary length $max_{len}$.

\State $Summ \gets []$
\State \textbf{PHASE 1} 
\While{$len(Summ) \leq g * max_{len}$}

    \State $Summ.append(topK(\{c(s_i^{I})\})$
\EndWhile \\
\State{\textbf{PHASE 2}} %\\
\While{$len(Summ) \leq max_{len}$}
\State $c(s_i^{I}) \gets c(s_i^{I}) - sim(c_{intra}(I), c_{intra}(J)) * \mu_2$ 
\Comment{J is the section index of last selected sentence, $\mu_2$ is a hyperparameter}
\State $Summ.append(top-1({c(s_i^{I})}))$
\EndWhile

\textbf{Return} Summ
\end{algorithmic}
\label{algorithm_1}
\end{algorithm}

Our approach can be divided into two phases, as shown in Algorithm \ref{algorithm_1}. In the first phase, we assume that important argumentative sentences at the two ends of the document can be easily detected (as shown in Figures \ref{fig:output_figure} and \ref{fig:three_view}, legal case documents generally start by introducing the issues and end with  conclusions).  A quantitative analysis of the top-5 selected sentences in CanLII in fact provides an 80\% coverage of issue or conclusion sentences.   We thus set up a threshold to pick the first k sentences based on the original document graphs. Afterward, we gradually downweight the sentence's centrality score using the location of the latest selected sentence, that is, we set a penalty score for sentences that are placed as a neighbor of the current sentence selected for the summary. Our rationale %behind such a procedure 
is that %we observe 
reasoning sentences are more likely to be located in different sections in the middle that are not shared with issues and conclusions. %As shown in Figure \ref{fig:three_view}, in legal cases the issues and conclusions are generally placed on the two ends of the article while the reasoning sentences are distributed in the middle. 
% \begin{table*}[h!]
% \small
% % \scriptsize 
%     \centering
%     % \setlength\tabcolsep{2.1pt}
%     \renewcommand{\arraystretch}{1}%Tighter
%     \begin{tabular}{c|l|ccc|ccc}
%     %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
%     \toprule
%       ID & Model  &  R-1 & R-2 & R-L  & BS \\
%          \midrule
%          \multicolumn{6}{c}{{Oracles}} \\
%          \midrule
%           1 & IRC & 57.92 & 35.72 & 55.05 &88.15 \\
%         2 &  EXT & 61.41 & 40.44 & 59.08 & 88.19 \\
          
%     \midrule 
%     \multicolumn{6}{c}{{Supervised Extractive }} \\
%     \midrule
%     3 & BERT\textsubscript{EXT} - selection & 40.78 & 17.63 & 37.75 & 84.05 \\
%     4 & SummRunnar & & & & \\
%      5 & SentCLR & & & & \\
%     \midrule
%     \multicolumn{6}{c}{{Supervised Abstractive}} \\
%     \midrule
%     6 & BART & 47.93 & 22.34 & 44.74 &  86.16 \\
%     7 & LED & 49.56 & 23.78 & 46.48  & 86.75\\
%     \midrule 
%         \multicolumn{6}{c}{{Unsupervised Extractive}} \\
%         \midrule 
%       8 & LSA & 38.15 & 18.22 & 35.76 & 84.63  \\
%           9& LexRank & 38.63 & 17.70 & 35.87 & 84.40 \\
%             10 & TextRank   & 36.70 & 16.19 & 34.00 & 83.53&  \\
%             11 & PACSUM & 39.24 & 14.31 & 36.80 & 81.64\\
%           \midrule 
%           \multicolumn{6}{c}{{HipoRank with different structures}} \\
%           \midrule
%                   12 & HipoRank (Original) & 43.42 & 18.04&  40.38 &  83.90 \\
%           13 & C99-topic & 42.03 & 16.89 & 39.32 &  83.59\\
%           14  & HMM-stage & 42.11 & 17.03 & 39.48 &  83.85 \\
%           \midrule 
%           15 & Original w/o header & 43.59 & 18.41 & 40.74 & 84.41 \\
%           16 & C99-topic w/o header & 44.32 & 18.57 & 41.50 & \textbf{84.56} \\
%           17 & HMM-stage w/o header & 43.76 & 18.52 & 41.07 & 84.53 \\
%           \midrule 
%         %   18 & Original Dynamic & 43.99 & 18.88 & 41.24 & 83.94\\
%         %   19 & C99-topic Dynamic & 43.76 & 18.25 & 41.04 & 83.81 \\
%         %     20 & HMM-stage Dynamic & 43.43 & 17.89 & 40.69& 83.93 \\
%         % \midrule 
    
%           18 & Original Dynamic + w/o H & 44.36 & 18.98& 41.63 &  84.43\\
%           19 & C99-topic Dynamic + w/o H & \textbf{45.33} & \textbf{19.77} & \textbf{42.54} & 84.50\\
%             20 & HMM-stage Dynamic + w/o H & 44.54 & 18.76 & 41.88 & 84.31 \\
%             \hline 
%             21 & C99-topic Dynamic + w/o H + sparse sent2sec & 44.84 & 19.28 & 42.07 & -- \\
%             \hline 
%             22 & Original Dynamic + w/o H + sent2sent reward & 44.18 & 18.86 & 41.37 & -- \\
%         \midrule
%     \bottomrule
%      \end{tabular}
%     \caption{Different Structure's Performance.}
%     \label{tab:unsupervised_results}
% \end{table*}

% \begin{table*}[h!]
% % \small
%     \centering
%     \renewcommand{\arraystretch}{1}%Tighter
%     \begin{tabular}{c|l|cc|cc}
%     %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
%     \toprule
%         & & \multicolumn{2}{c}{\textbf{CanLII}} & \multicolumn{2}{c}{\textbf{BillSum}} \\
%       ID & Model  &  R-1/R-2/R-L  & BS & R-1/R-2/R-L  & BS\\
%          \midrule
%          \multicolumn{6}{c}{{Oracles}} \\
%          \midrule
%           1 & IRC & 58.04/36.02/55.28 & 87.94 & N/A & N/A \\
%         2 &  EXT (ROUGE-L, F1) & 59.38/38.77/56.94 &87.85  & 56.04/37.50/53.10 & 87.30\\
        
   
          
%     \midrule 
%     \multicolumn{6}{c}{Baselines} \\
%     \midrule
%     \multicolumn{6}{l}{\textit{supervised}} \\
%     % 3 & BERT\textsubscript{EXT} - selection & 40.78 & 17.63 & 37.75 & 84.05 \\
%     3 & BERT\_EXT & \textit{43.44}/\textit{17.84}/\textit{40.36} & \textit{84.47} & 39.57/15.89/35.08 &  83.54 \\
%     %  5 & SentCLR & & & & \\
%     % \midrule
%     % \multicolumn{6}{c}{{Supervised Abstractive}} \\
%     % \midrule
   
%     % 6 & BART & 50.50/25.58/46.82 &  87.25& \\
%     % 7 & LED & 53.72/28.75/ 50.17 & 87.55&\\
%     % \midrule 
%         \multicolumn{6}{l}{\textit{unsupervised}} \\
%         % \midrule 
%       4 & LSA & 37.22/17.82/34.87 & \underline{\textit{84.48}} & 40.44/18.07/36.31 &  83.70 \\
%           5 & LexRank & 37.90/\underline{\textit{18.17}}/35.62 &  84.32 &  41.26/\textbf{\underline{\textit{21.19}}}/37.43 & 84.02\\
%             6 & TextRank  & 36.70/16.19/34.00 & 83.51 & 36.38/16.93/30.84 & \textbf{\textit{\underline{84.49}}}\\
%             7 & PACSUM & 40.01/15.68/37.37 & 83.52  & 40.71/18.23/37.00 & 83.08  \\
%             8 & HipoRank (Original Structure) &  \underline{41.61}/17.13/\underline{\textit{38.73}}  & 83.55  & \underline{\textit{42.41}}/19.48/\underline{\textit{38.65}} & 83.24 \\
%           \midrule 
%           \multicolumn{6}{c}{{Document Structure with HipoRank backbone}} \\
%           \midrule
%                 %   12* & Original 
%           9 & C99-topic & 41.33/16.48/38.45 &  83.53 & 41.82/18.62/37.94& 83.57 \\
%           10  & HMM-stage & 40.71/15.64/37.93 & 83.57 & \textbf{42.97}/{20.37}/\textbf{39.24} & {83.90} \\
%         %   \midrule 
%           11 & Original Structure w/o header & 42.56/17.96/39.62 & 83.62 & N/A & N/A \\
%         %   & Original w/o header + truncation & 42.85/17.46/39.88 \\ 
%           12 & C99-topic  w/o header & 43.25/18.02/40.25 & \textbf{84.48} & N/A & N/A   \\
        
%           13 & HMM-stage  w/o header & 42.64/17.38/39.76 & 83.57 & N/A & N/A \\
          
%           \midrule 
%               \multicolumn{6}{c}{{Document Structure with HipoRank backbone + reweighting Algorithm}} \\
%               \midrule
%           14 & Original Structure* & 43.18/{18.35}/40.26 &  84.20  & 42.30/19.73/38.69 & 83.11 \\ 
%           15 & C99-topic* & \textbf{43.89}/\textbf{18.67}/\textbf{41.00} &  {84.34} & 40.78/17.95/37.02 & 83.15\\
%             16 & HMM-stage* & {43.28}/17.80/40.40 &  84.22 & 42.09/19.83/38.48 & 83.56\\ 
%             % 17 & Ours + sentence\_relation & 43.26/18.33/40.38 & \\
            
%         \midrule
%     \bottomrule
%     \end{tabular}
%     \caption{The automatic evaluation results on CanLII and BillSum test sets, \textbf{bold} represents the best non-oracle extractive score, \textit{italic} for the best baselines and \underline{underline} for best unsupervised baseline. Model name with stars, we use the without header version of CanLII dataet as input and keep the original BillSum data.} % need to make sure the notation is obvious. 
%     \label{tab:unsupervised_results}
% \end{table*}


==> EMNLP -- Legal Summarization-3/Sections/RelatedWork.tex <==
\section{Related Work}

% \subsection{Controllable Summary Generation}
% Controllable generation can be described as methods to control a language model’s text generation given some kind of guidance. Work has focused on several aspects such as the summary length \cite{liu-etal-2018-controlling, fan-etal-2018-controllable, saito2020length}, styles \cite{zhang-etal-2018-shaped, jin-etal-2020-hooks} or via prompting \cite{he2020ctrlsum}. \citet{song-etal-2021-new} introduced a two-stage approach to first generate
% multiple summaries, then applying filters to select the summary with
% the desired style or property. \citet{goyal2021hydrasum} further utilize multiple
% decoders which specialized in different stylistic features into a transformer framework. These approaches focused on controlling certain style aspects of the text. On the other hand, \cite{dou-etal-2021-gsum} recently proposed a framework to incorporate extra guiding signals like keywords or salient sentences into the summarization models. Different from previous work, instead hinting the model with extra signals for better content selection, our approach aims at generating summaries with explicitly controlled discourse structure, that can be learned from the reference summary.

%\subsection
{\bf Supervised Extractive Summarization Using Discourse Information}
Graph-based methods have been exploited for extractive summarization tasks to better model the inter-sentence relations based on document structure. \citet{xu-etal-2020-discourse} applied a GCN layer to aggregate information from the document's discourse graph based on RST trees and dependencies.  More recently, 
 HiStruct+ \cite{ruan-etal-2022-histruct} and HEGEL \cite{zhang-2022-hegel} started to incorporate the hierarchical structure and topic structure of scientific articles into supervised model training, respectively. However, HiSruct+ relied on the relatively fixed and explicit document structure of scientific articles\footnote{Section titles following a shared pattern (introduction, method … and conclusion) are encoded to provide structural information. However, in our dataset, sectioning is often missing 
 %– 297 test articles do not come with split paragraphs – or do not come with meaningful section titles %
 or not meaningful (e.g.,  titles such as "section 1").},
 %(i.e., some legal documents have section titles of ``section 1'', ``section 2'', etc.)},
 while HEGEL relied on a large training set to identify the topic distributions. \textit{Our work uses an unsupervised extractive summarization approach in a lower-resource setting, as well as studies the effects of computing different types of document structures.}
 We leave the exploration of the aforementioned supervised approaches on legal domain texts for future work.  
%\subsection

{\bf Unsupervised Extractive Summarization}
Traditional extractive summarization methods are mostly unsupervised \cite{radev-etal-2000-centroid, 10.5555/2832415.2832442,  hirao-etal-2013-single}, where a large portion apply the graph-based algorithms \cite{SALTON1997193, Steinberger2004UsingLS,erkan2004lexrank} or are based on term frequencies such as n-gram overlaps \cite{Nenkova2005TheIO} to rank the sentences' importance. More recently, pretrained transformer-based models \cite{devlin-etal-2019-bert, lewis-etal-2020-bart, zhang2020pegasus} have provided better sentence representations. %for unsupervised summarization 
%\cite{zheng-lapata-2019-sentence, dong-etal-2021-discourse}. 
For instance, \citet{zheng-lapata-2019-sentence} built directed unsupervised graph-based models on news articles using BERT-based sentence representations and achieved comparable performance to supervised models on multiple benchmarks. \citet{dong-etal-2021-discourse} %further 
augmented the document graph of \citet{zheng-lapata-2019-sentence}
with sentence position and section hierarchy to reflect the
document structure of scientific articles. \textit{Different from these two works which are based on assumptions of news and scientific article structures, our method uses reweighting to better utilize the document structure of legal cases.}

%\subsection
{\bf Extractive Summarization of Legal Texts}
%Extractive summarization of legal case documents remains a practical challenge.
Despite the success of supervised neural network  models in news and scientific article summarization \cite{zhang2020pegasus, lewis-etal-2020-bart,zaheer2020bigbird}, they face challenges in legal document summarization given the longer texts, distinct document structure, and limited training data \cite{bhattacharya2019comparativestudy}. Instead, prior work has tackled legal extractive summarization by applying domain independent unsupervised algorithms \cite{Luhn-1958-automatic,erkan2004lexrank,  sarvanan-2006-graphical}, or designing domain specific supervised approaches \cite{sarvanan-2006-graphical, polsley-etal-2016-casesummarizer,zhong-2019-iterativemasking}. One recent work \cite{bhattacharya2021incorporating} frames the task as Integer Linear Programming and demonstrates the importance of in-domain structure and legal knowledge. %while comparing to general supervised models such as \textsc{SummaRuNNer} \cite{nallapati2017summarunner} and \textsc{BertSum} \cite{liu-lapata-2019-text}. 
In another line of research, \citet{xu-2021-position-case} propose a sentence classification task with the hope of exploiting the court decision's \textit{argument structure} by making explicit its issues, conclusions, and reasons (i.e., argument triples). \textit{Our work is unsupervised
%does not require supervised training process 
and implicitly reveals the relations between argument triples to generate better summaries.}

==> EMNLP -- Legal Summarization-3/Sections/Unsupervised_Generation.tex <==

% \section{Unsupervised Summarization}




\section{Experimental Setup}
%We discuss the evaluation metrics and other models  used in our experiments. 
For supervised models, we split the training data in an 80:20 ratio for training and validation. For unsupervised models, we tune the hyperparameters on the validation set. Model training details can be found in Appendix \ref{appendix:detail}. 

% \subsection{Datasets}
% Our experiments are conducted on CanLII \cite{} and
% BillSum \cite{kornilova-eidelman-2019-billsum}, two large-scale datasets
% of long and structured legal documents with human-written summaries. The average source article
% length is xxxx and 1382 tokens, making them ideal
% candidates to test our method.

%\subsection{Oracle and Baseline Models}



\begin{table*}[t]
% \small
    \centering
    \renewcommand{\arraystretch}{1}%Tighter
    \begin{tabular}{c|l|cccc}
    %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
    \toprule
  %      & & \multicolumn{2}{c}{\textbf{CanLII}} \\
      ID & Model  &  R-1 & R-2 & R-L   & BS\\
         \midrule
         \multicolumn{6}{c}{{Oracles}} \\
         \midrule
          1 & IRC & 58.04 & 36.02 &55.28 & 87.94  \\
        2 &  EXT (ROUGE-L, F1) & 59.38 & 38.77 & 56.94 & 87.85 \\
        
   
          
    \midrule 
    \multicolumn{6}{c}{Extractive baselines (no document structure)} \\
    \midrule
    \multicolumn{6}{l}{\textit{supervised}} \\
    % 3 & BERT\textsubscript{EXT} - selection & 40.78 & 17.63 & 37.75 & 84.05 \\
    3 & BERT\_EXT & \textit{43.44} & {17.84} & \textit{40.36} & {84.47}  \\
    %  5 & SentCLR & & & & \\
    % \midrule
    % \multicolumn{6}{c}{{Supervised Abstractive}} \\
    % \midrule
   
    % 6 & BART & 50.50/25.58/46.82 &  87.25& \\
    % 7 & LED & 53.72/28.75/ 50.17 & 87.55&\\
    % \midrule 
        \multicolumn{6}{l}{\textit{unsupervised}} \\
        % \midrule 
       4 & LSA & 37.22 & 17.82 & 34.87 & {\bf \underline{\textit{84.48}}} \\
           5 & LexRank & 37.90 &\underline{\textit{18.17}} & 35.62 &  84.32 \\
            6 & TextRank  & 36.70 &16.19 &34.00 & 83.51 \\
            7 & PACSUM & 40.01 & 15.68 &37.37 & 83.52  \\
            %8 & HipoRank (Original Structure) &  \underline{41.61} & 17.13 & \underline{\textit{38.73}}  & 83.55  \\
           \midrule 
           \multicolumn{6}{c}{{HipoRank backbone (with different computed document structures) 
           %with HipoRank backbone
           }} \\
          \midrule
                %   12* & Original 
          8 & Original Structure &  {41.61} & 17.13 & {38.73}  & 83.55  \\
          9 & C99-topic & 41.33 & 16.48 & 38.45 &  83.53  \\
          10  & HMM-stage & 40.71 & 15.64 & 37.93 & 83.57 \\
        %   \midrule 
          11 & Original Structure w/o header & 42.58 & 18.01 & 39.63 & 83.62 \\
        %   & Original w/o header + truncation & 42.85/17.46/39.88 \\ 
          12 & C99-topic  w/o header & \underline{43.25} & 18.02 & \underline{40.25} & \underline{\textit{\textbf{84.48}}} \\
        
          13 & HMM-stage  w/o header & 42.64 & 17.38 & 39.76 & 83.57\\
          
          \midrule 
              \multicolumn{6}{c}{{Ours (HipoRank backbone + Reweighting Algorithm)}} \\
              %Document Structure with HipoRank backbone + reweighting Algorithm}} \\
              \midrule
          14 & Original Structure w/o header & 43.14 & {18.46} & 40.23 &  84.20  \\ 
          15 & C99-topic w/o header & \textbf{43.90} & \textbf{18.67} & \textbf{41.00} &  {84.34} \\
            16 & HMM-stage w/o header & {43.28} & 17.80 &40.40 &  84.22 \\ 
            % 17 & Ours + sentence\_relation & 43.26/18.33/40.38 & \\
            
        \midrule
    \bottomrule
    \end{tabular}
    \caption{The automatic evaluation results on the CanLII test set. \textbf{Bold} represents the best non-oracle score, \textit{italic} the best baseline/backbone score, and \underline{underline} the best unsupervised baseline/backbone score.} %The model names with "w/o header" use the without header version of CanLII dataet as input to .} % need to make sure the notation is obvious. 
    \label{tab:unsupervised_results}
\end{table*}

\textbf{Upper Bound Oracles}\label{sec:oracle}  %Taking advantage of the annotations in our test set and 
Based on  Figure \ref{fig: disbribution}, we create a domain-dependent \textbf{IRC\_Oracle} model where test sentences  manually annotated with the IRC  labels are concatenated to form the summary.   Following \citet{nallapati2017summarunner}, we also report results for \textbf{EXT\_Oracle}, a domain-independent
summarizer %\cite{nallapati2017summarunner}, 
which greedily selects sentences from the original document based on the ROUGE-L scores compared to the abstractive human summary. %This model selects sentences whose concatenation maximizes the evaluation metric given the gold summary.

\textbf{Extractive Baselines} %We compare our proposed discourse views and reweighting algorithm with various baselines. 
For unsupervised models, we compare with LSA  \cite{Steinberger2004UsingLS},
LexRank \cite{erkan2004lexrank}, TextRank \cite{DBLP:journals/corr/BarriosLAW16}, and PACSUM \cite{zheng-lapata-2019-sentence}. We also include HipoRank \cite{dong-etal-2021-discourse} with document views. %),  as it achieved high %the state of the art 
%performance on long scientific papers.  %summarization
For supervised methods, we compare with BERT\_EXT \cite{liu-lapata-2019-text}. % uses a  document-level encoder based on BERT. % which is able to express the semantics of a document and obtain sentence representations. 
Although not our focus,  abstractive baselines are in Appendix \ref{sec:appendix_abstractive}. 

%\subsection
\textbf{Automic Evaluation Metrics}
%For automatic evaluation, 
We report ROUGE-1 (R-1), ROUGE-2 (R-2), and ROUGE-L (R-L) F1 scores, as well as % We also report
BERTScore (BS) \cite{bert-score}. %to measure the semantic meanings of the generated summary. 
%Finally, we design an automatic metric for the CanLII dataset. 
%Recall from Section  \ref{sec:dataset} that our test set comes with sentence-level annotations on both source and target texts following the ``IRC'' scheme. %, that is, a sentence can be manually classified as either Issue, Reason, Conclusion or Non-IRC types. %(more detailed description in \S \ref{sec:dataset}). 
We also propose metrics to measure the recall value of the annotated IRC types in the test set, % in source-side, as well as the recall values in the summary, 
which exploits the structure of case documents. More details are in Section \ref{sec:salient_eval}.  

 
     
\section{Results}\label{sec:result}
In this section, we aim to deal with three research questions: 
\textbf{RQ1}. How well do the extractive baselines including the HipoRank backbone deal with legal documents?  
\textbf{RQ2}. How well do the different views of document structures perform with the  HipoRank backbone?  \textbf{RQ3}. Can the reweighting algorithm help select important argumentative sentences and improve summary quality?

\subsection{Automatic Summarization Evaluation}
Table \ref{tab:unsupervised_results}
% We 
compares our methods with prior extractive models. See Appendix \ref{appendix:output} for example summaries. % can be found %in Appendix \ref{appendix:output}. 
% The first block in Table \ref{tab:unsupervised_results} includes the IRC 
%and the extractive oracles. The next
%block  presents the results of one supervised
%and several unsupervised extractive
%baseline models. The block after that presents the discourse-aware HipoRank baseline with our different views of document structure.  The final block presents our reweighting  model's results (using the "w/o header" version of the CANLLI documents as they performed best in the prior block.) 


%Overall, our approach on incorporating the different document views and selection methods obtained the best results on the datasets.

\textbf{RQ1.} Table \ref{tab:unsupervised_results} shows that there is still a gap between oracle models (rows 1 and 2) and current extractive baselines. There are around 20 points differences on R-1, R-2, and R-L. Among the baselines, the supervised model works best  only for R-1 and R-L. Unsupervised methods obtain  the highest BS (row 4) and R-2  (row 5), possibly due to the higher coverage of n-grams benefitting from longer extracted summaries (row 3 model generated summaries have an average length of 250; row 4-6 models generate on average 400-word summaries;  row 7 and 8 models have a limit of 220 words). %Comparing to the supervised model, unsupervised methods (row 4-8) have lower scores, which is reasonable given that the model is not exposed to any training data.
Without  reweighting, the HipoRank backbone % - even with the best performing document structure - 
never outperforms the best extractive baseline.  However, if only unsupervised baselines are considered,  HipoRank in row 12 does show the best performance for 3 of the 4 evaluation metrics.
%We first compare the best-performed baseline model, HipoRank's performance given documents with different structure representation. 

\textbf{RQ2.} To examine the effects of the  document views in  Section \ref{sec:views}, we split the document into different types of linear segments and then used  HipoRank  to generate summaries.  Recall that HipoRank is the only model to exploit  document structure, and as noted for RQ1, with the right structure could obtain the  best unsupervised R-1, R-L, and BS baseline scores.  
When naively constructing different document structures from the CanLII dataset without header removal, using NLP algorithms (rows 9 - 10) versus just using the HTML formatting (row 8) generally degraded results. However, when we  experimented with a modified version of the input documents (rows 11-13) where the headers were filtered through heuristics before computing the document structure, %and keyword matching and sections are reorganized 
%(see Section \ref{sec:header_removing}), %the C99 model (row 12) outperformed just using the HTML (row 11).  In addition, 
the  scores in rows 11-13 were higher (or in one case the same) than the comparable scores in rows 8-10.  
Also, without headers, the C99  topic segmentation algorithm (row 12) now outperforms the use of HTML (row 11) (obtaining an average improvement of 0.5 points across ROUGE and 0.8 for BS), suggesting
 that better  structures can  improve summarization. 
% As shown in row 11-12 in third block of Table \ref{tab:unsupervised_results}, the original document structure outperforms the other two views on the CanLII dataset and HMM-Stage obtains best performance on BillSum. 
% Through visualization of the IRC and selected sentence positions in the CanLII document (Fig \ref{fig:initial_study}), 
% we find that the stage-based segmentation perform better on selecting sentences appeared in the middle of the text (green ovals in the bottom right sub figure) while the topic-focused one succeeded in more accurately capturing the ending "conclusion" sentences (two green ovals in top-left sub figure). 
% \begin{figure}
% \centering
%  \includegraphics[width=\linewidth]{Figs/1654088145579.jpg}
%   \caption{Initial study on selected sentence positions from different views.}
%   \label{fig:initial_study}
% \end{figure}
 As shown in Table \ref{tab:segmentation_stats} (and earlier in Figure \ref{fig:three_view}), C99  creates many small sections (average number of sentences per section is 3.39 with standard deviation  of 0.67).
 We hypothesize that this encourages the selection of sentences from more fine-grained segments. In contrast, the other two methods create lengthy sections (average of more than 50 sentences) with a large standard deviation (135.40 for original structure without headers). 
%Also, the C99 model (row 12) now outperformed just using the HTML (row 11)
% With the updated CanLII dataset, we find that changing to different document structure, such as the topic segmentation, we 
In sum, with improvements in automatic metrics, we find that document structures play an important role in summarizing cases.
\begin{table}[t]
\small
    \centering
    \begin{tabular}{c|c|c}
    \toprule
        Model & avg. \# secs & avg. \# sents per sec  \\
        \midrule 
        \multicolumn{3}{c}{with header} \\
        \midrule
        Original Structure & 4.83 (6.44) &  83.82 (118.78) \\
        C99-topic & 63.47 (70.34) & 3.38 (0.71) \\
        HMM-stage & 4.00(0.83) &  54.32 (64.80) \\
        \midrule
         \multicolumn{3}{c}{without header} \\
         \midrule
        Original Structure & 3.67 (5.51) &  102.99 (135.40) \\
        C99-topic & 59.74 (69.91) & 3.39 (0.67) \\
        HMM-stage & 3.16 (1.08) &  70.19 (119.39)\\
        \bottomrule
    \end{tabular}
    \caption{Statistics about the average number of sections (avg. \# secs) and average number of sentences per section (avg. \# sents per sec) across the documents with different computed document structures (standard deviation in parenthesis).}
    \label{tab:segmentation_stats}
\end{table}

\textbf{RQ3}. The final block of Table \ref{tab:unsupervised_results} presents the reweighting  results (using the "w/o header" version of the CanLLI documents as they performed best in the prior block).  %We first implement the reweighting algorithm. 
By downweighting  sentences that appear under the same section as  previously selected ones, we observe an F1 improvement of 0.65, 0.65, and 0.75 on R-1, R-2, and R-L, respectively, on the previously best-performing topic segmented document (row 12 versus 15).
%Employing HipoRank with C99-topic segmentation and adding our reweighting algorithm 
Row 15 in fact has the best non-oracle results for all ROUGE scores.  This observation regarding the value of reweighting also holds for the original structure (row 11 vs. 14) and the HMM-stage segments (row 13 vs. 16). %\footnote{For ROUGE precision and recall, see Appendix \ref{appendix:viewFullResults}.}
%Overall, our approach gives an improvement of 2.2 on R-1, 1.5 on R-2 and 2.3 on R-L on the CanLII dataset (row 8 and row 15).   %Interestingly, the  proposed selection algorithm bring negative results on the BillSum dataset, an analysis on the position distribution of the extractive oracle sentences (see Figure \ref{fig:billsum_position_sorted} in Appendix) in the original article demonstrated that the salient information in the original article are following a uniform distribution, thus the proposed algorithm may discourage for better selection of candidates. 

% \begin{figure*}
% % \begin{adjustwidth}{-8em}{0em}
%   \begin{subfigure}[b]{0.7\textwidth}
%     \includegraphics[width=\textwidth]{Figs/Oracle_IRC_no_sort.png}
%     \caption{IRC Oracles}
%     \label{fig:}
%   \end{subfigure}
%   %
%   \begin{subfigure}[b]{0.7\textwidth}
%     \includegraphics[width=\textwidth]{Figs/positions_test_pacsum_no_order.png}
%     \caption{PacSum}
%     \label{fig:}
%   \end{subfigure}

%   \begin{subfigure}[b]{0.7\textwidth}
%     \includegraphics[width=\textwidth]{Figs/positions_test_hiporank_no_order.png}
%     \caption{HipoRank}
%     \label{fig:}
%   \end{subfigure}
%   %
%   \begin{subfigure}[b]{0.7\textwidth}
%     \includegraphics[width=\textwidth]{Figs/positions_test_theme1_1049_dynamic_no_order.png}
%     \caption{Ours}
%     \label{fig:}
%   \end{subfigure}
% \end{figure*}

\begin{figure*}[h]
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/Oracle_IRC_no_sort.png}
            \caption[]%
            {{\small IRC Oracles}}    
            \label{IRCoracle}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.45\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{Figs/positions_test_hiporank_no_order.png}
            \caption[]%
            {{\small HipoRank with headers}}    
            \label{fig:mean and std of net34}
        \end{subfigure}
        \vskip\baselineskip
        
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/positions_test_1049_noheader.png}
            \caption[]%
            {{\small HipoRank without headers}}    
            \label{IRCoracle}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.45\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{Figs/positions_test_1049_noheader_dynamic.png}
            \caption[]%
            {{\small HipoRank without headers and with reweighting}}    
            \label{fig:mean and std of net34}
        \end{subfigure}
        \vskip\baselineskip
        %%%%%%%
        % \hfill
        % \begin{subfigure}[b]{0.485\textwidth}   
        %     \centering 
        %     \includegraphics[width=\textwidth]{Figs/positions_test_1049_noheader.png}
        %     \caption[]%
        %     {{\small HipoRank without headers}}    
        %     \label{fig:mean and std of net44}
        % \end{subfigure}
        % % \vskip\baselineskip
        % \hfill
        % \begin{subfigure}[b]{0.485\textwidth}   
        %     \centering             \includegraphics[width=\textwidth]{Figs/positions_test_theme1_1049_dynamic_no_order.png}
        %     \caption[]%
        %     {{\small Our with Reweighting}}    
        %     \label{fig:mean and std of net44}
        % \end{subfigure}
        
        \caption[]
        {\small Sentence positions in source cases for extractive summaries generated by different models using the original document structure on the
 test set. For (b) (c) (d), documents on the x-axis are
sorted in the same order. For IRC Oracles, \textcolor{red}{Issue}, \textcolor{reasonblue}{Reasoning} and \textcolor{conclusiongreen}{Conclusion} sentences are colored accordingly. } 
        \label{fig:comparison}
    \end{figure*}
    
    Finally, to better understand the behavior of different enhancements to the HipoRank backbone model, Figure \ref{fig:comparison} visualizes the positions of IRC sentences in the original article that are selected by a particular summarization method.  Plot (a) shows that the human-annotated IRC sentences in the summary tend to span across the source documents, with issues appearing in the beginning and conclusions in the end. Plot (b) shows that although HipoRank using the original document structure can successfully pick middle section sentences, the darkest band at the starting positions shows that the model still heavily relies on the inductive bias to pick the beginning sentences. Plot (c)
shows that removing the headers reduces the  starting sentence bias.  Finally, plot (d) shows that 
%We find that 
reweighting  reduces the number of sentences appearing on both ends. Further analyses on the complete automatic evaluation results\footnote{See Appendix \ref{appendix:reweight_effects} for ROUGE precision and recall.} suggest that the improvements come from higher recall values.
%(as shown in Fig \ref{fig:comparison}). 


\subsection{Argumentative Sentence Coverage}\label{sec:salient_eval}
Taking advantage of the sentence-level IRC annotations, we propose recall metrics to better measure the summary quality from a legal argumentation perspective ({\bf RQ3}).  We compute the recall of ``IRC'' sentences extracted from the original case as source IRC coverage (src. IRC). % of the summarizer. 
We similarly compute the coverage of IRC sentences in the human-written summaries as target IRC coverage (tgt. IRC) and all sentences as target sentence coverage (trg. cov.). To do so we apply the oracle summarizer (Section \ref{sec:oracle}) to map the generated extractive summaries to the human-written abstractive summaries. % and report the corresponding recall values. 

%\footnote{This oracle summarizer obtains a recall of 84.0 on the IRC mappings among the case and human written summaries manually annotated on ten article pairs.} 

We report these values for the IRC oracle, %the best 
an unsupervised (LexRank) and supervised (BERT\_EXT) baseline, the  discourse-aware HipoRank with the original structure, and our best reweighting model using C99-topic segmentation. Table \ref{tab: salient_coverage} shows that our model obtains the highest target IRC recall and coverage, suggesting that the  summaries are more similar to the references with respect to %conveying 
the decision's argumentation. Another unsupervised model, LexRank, obtains the highest source IRC, but its off-the-shelf package requires a fixed sentence ratio selected from the source. %original article. 
This produced longer summaries than other approaches and thus captured more IRCs in the source. 

\begin{table}[t!]
\small
    \centering
    \renewcommand{\arraystretch}{1}%Tighter
    \begin{tabular}{c|c|c|c}
    %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
    \toprule
  \textbf{Model} & \textbf{src. IRC} & \textbf{tgt. IRC} & \textbf{trg. cov.} \\
  \midrule 
  \multicolumn{3}{l}{\textit{Oracle}}\\
  \midrule
  IRC & 1 (0.00) & 0.918 (0.18)  &  0.820 (0.25) \\
%   EXT &   62.7 & 71.7 & 66.3  \\
  \midrule 
     \multicolumn{3}{l}{\textit{Baselines}}\\
  \midrule
  BERT\_EXT & 0.804 (0.27) & 0.846 (0.23) &  0.833 (0.23)\\
  LexRank & \textbf{0.912} (0.19) & 0.811 (0.26) &  0.800 (0.27)\\
%   PACSUM & & \\
  HipoRank & 0.800 (0.25) & 0.851 (0.24) & 0.844 (0.22) \\
   
  \midrule 
  {\it Ours} & 0.823 (0.26) & \textbf{0.866} (0.20) & \textbf{0.850} (0.21) \\
  \bottomrule

    \end{tabular}
    \caption{Average recall of IRC sentences matched in the original case (src. IRC), gold summary (tgt. IRC), as well as target sentences coverage (trg. cov.) for each document (standard deviation in parenthesis).}
    \label{tab: salient_coverage}
\end{table}


\subsection{Human Evaluation Discussion}
% TODO: add the newest paper citation.

% Another limitation is that current references are fixed, which could not address the prior work's expert feedback that there is a need for different kinds of summaries in the legal field, depending on the expert's intention of use.  

As a first step towards human evaluation, we tried to extend the HipoRank  setup in \citet{dong-etal-2021-discourse} and designed a human evaluation protocol as follows. We asked human judges\footnote{All judges should be native English speakers who are at least pursuing a JD degree in law school and have experience in understanding case law.} to read the human-written reference summary and presented  extracted sentences from different summarization systems. The judges were asked to evaluate a system-extracted sentence according to two criteria: (1) \textit{Content Coverage} -  whether the presented sentence contained content from the human summary, and (2) \textit{Importance} - whether the presented sentence was important for a goal-oriented reader even if it was not in the human summary\footnote{Here we assumed the goal-oriented reader as the lawyers or law students seeking information from the case.}. The sentence selection was anonymized and randomly shuffled. We used the same sampling strategy in \citet{dong-etal-2021-discourse} to pick ten reference summaries where the system outputs were neutral (i.e., had similar R-2 scores compared to the human reference). 
%The evaluators also provide valuable feedback on keeping track of the metadata about annotators' legal backgrounds, area specialization, and experience with lawsuits. 
However, initial annotation on a small set by a legal expert demonstrated that the selected sentences may not reflect the model's capability. Most sampled system outputs had low ROUGE-2 F1 scores compared to the reference (normally below 10\% while the average model performance is 17\%), and the human evaluator reported that some of the selected sentences were not meaningful. We thus propose that a more careful sampling technique will be required for legal annotation tasks such as ours. 

To further guide our future work, we also reviewed how prior legal domain research has performed human evaluations when automatically summarizing legal documents  \cite{polsley-etal-2016-casesummarizer, zhong-2019-iterativemasking, salaun-2022-jurix}. Due to the burden of reading lengthy original documents, as in our human evaluation, most prior work evaluated summary quality using reference summaries rather than  source documents. In addition,  legal evaluations have typically been small-scale %constrained by the scale 
(5-20  summaries) due to the need to have evaluators with particular types of expertise (e.g., law graduate students or law professors), which was a similar constraint in our exploratory human evaluation.  Researchers have also designed new types of legally-relevant evaluation questions that  evaluate the summary for task-specific properties that go beyond more typical properties such as grammar, readability, and style. In our case, we would like legal experts to assess IRC coverage in the future.

% In caseSummarizer, \citet{polsley-etal-2016-casesummarizer} recruited domain-experts (without further details) and designed a tiny scale of (5 summaries) human evaluations with six questions borrowed from meeting summarization \cite{5071230}. \citet{zhong-2019-iterativemasking} recruited a law professor to examine different system outputs of 20 cases with a single question ``whether the summary adequately identifies issues and resolutions''. More recently, in \cite{}, SALAUN three experts (nlp specialist and law graduate students) annotated 16 test instances with an intrinsic evaluation framework of 7 questions to evaluate the summary from the form properties (grammar, readability, and style) and summary adequacy properties. Despite the small scale, most prior attempts avoided including the original long cases, given the time expense and difficulty in capturing all details, and instead focused on comparing the summaries to the references. Such evaluations may not be able to address the sentence-level properties of the extracted summaries.

% \textcolor{blue}{For this task, to evaluate the selected sentences' quality, following the work of \citet{dong-etal-2021-discourse}, we design a human-evaluation protocol as follows:  to read the human-written reference summary and present those extracted sentences from different summarization systems. The judges are asked to evaluate the system-extracted sentence according to two criteria: (1) \textit{Content Coverage}  whether the presented sentence contains content from the human summary and (2) \textit{Importance} whether the presented sentence is important for a goal-oriented reader even if it is not in human summary\footnote{Here we assume the goal-oriented reader as the lawyers or law students seeking information from the Case.}. The sentence selection is anonymized and randomly shuffled, so the human judges will not know which system it comes from. Given that the total amounts of sentences are too large (each system summary can have 10-20 sentences), it is infeasible to annotate all sentences of the 1,049 test cases. We instead try to sample a small portion of the data. As did in \cite{dong-etal-2021-discourse}, we selected ten reference summaries coupled with a total of 281 system-extracted sentences, where 141 are from our best model (row 15 in Table \ref{tab:unsupervised_results}) and 141 from the hiporank baseline with original structure (row 11 of Table \ref{tab:unsupervised_results}). Criteria are applied for the selection, where both system outputs have similar ROUGE scores compared to the human reference but differ dramatically from each other for neutral comparison. However, initial annotation on a small set from the 281 tasks demonstrates that the selected sentences may not represent the whole dataset. Most sampled system outputs have low ROUGE-2 scores compared to the reference (normally below 10\%), and human evaluators also report that some of the selected sentences are not good enough. We thus propose that a more careful sampling technique is required for the annotation tasks of the legal domain. The evaluators also provide valuable feedbacks on keeping track of the metadata about annotators' legal background, the specialization of area, and the experience with lawsuits.  }



% TODO: (1) Ablation Study on different views' selected results and the way to aggregate. (2). Examine the strategies to weight different section-sentence edges. (3) show different variants of the multi-round revision and demonstrate the benefits. 



==> EMNLP -- Legal Summarization-3/arxived/Controlled_Generation_Experiment_Setup.tex <==
\section{Controllable Summary Generation}
We frame the controllable summary generation as a natural language generation task. We compare our proposed approach with multiple baselines for both extractive and abstractive summarization in \S \ref{sec:result} using multiple automatic metrics. We find that the structure aware summary generation outperforms vanilla models. We additionally propose a salient rewarding metrics that can more precisely evaluate the coverage and adherence of generation result while giving the user provided prompt.

\subsection{Structure Guided Summary Generation}
From the corpus released by (cite Huihui's newest paper),  annotators are asked to annotate individual sentences in the summary following the IRC schema (described in \S dataset). Thus, the annotated data comes with a label sequence which represents the structure of the summary. One example can be found in Figure \ref{}. For the abstractive summarziation models, we add the annotated text sequence before the original texts, thus letting the model to implicitly map the structure sequence to the generation summary sentences.

% \subsection{Long Input Split}
% Most neural extrative summarizers are limited by the length of inputs, which is usually 512 tokens cite{BERT} and fall far below the average length of 5k tokens in the legal documents. It is impractical to concatenate all sentences in a document and encode them with a large pretrained model. Following \cite{mao2021dyle}, we group consecutive sentences into \textit{chunks}. We set the maximum length at 512 and allow for 20\% overlapping with the previous chunk. This way we could include the intermediate sentences in multiple chunks, wishing to capture local dependencies within the same section or paragraph. 

\subsection{Extractive Summarization}
\paragraph{Extractive oracles.} \textit{Extractive oracles} denotes a set of selected text snippets whose concatenation maximizes the evaluation metric given the gold summary. We first utilize the \textbf{IRC\_Oracle}, which sentences manually labelled with the IRC types are concatenated together to form a extractive summary. Following \cite{nallapati2017summarunner}, we additionally report \textbf{EXT\_ORACLE}, a baseline for an
oracle summarizer \cite{nallapati2017summarunner}, which greedily select sentences from the original article based on the ROUGE-L scores comparing to the abstractive summary.

\paragraph{Extractive Baselines}
We compare the proposed framework with various baselines. For unsupervised extractive summarization models, we compare with LSA  \cite{Steinberger2004UsingLS},
LexRank \cite{erkan2004lexrank}, TextRank \cite{DBLP:journals/corr/BarriosLAW16}, PACSUM \cite{zheng-lapata-2019-sentence}. We further include HipoRank \cite{dong-etal-2021-discourse}, which achieved the state of the art performance on scientific paper summarization, which also has long text inputs.
For supervised methods, BERTEXT \cite{liu-lapata-2019-text} uses a novel document-level encoder based on BERT which is able to express the semantics of a document and obtain representations for
its sentences. 

\subsection{Abstractive Summarization}
For abstracive summarization, we experiment with BART \cite{lewis-etal-2020-bart} and the Longformer-Encoder-Decoder (LED) \cite{Beltagy2020Longformer}. The latter model can process longer input document up-to 16k tokens. 

\subsection{Implementation Details}
For PACUSUM, we used the released bert checkpoint\footnote{\url{https://github.com/mswellhao/PacSum}}.For BERTEXT without fine-tuning, we use the released checkpoint\footnote{https://github.com/nlpyang/PreSumm} trained on CNN$/$DailyMail Dataset and inference the extracted sentence from each chunk. One limitation of training the BERTEXT model is that the BERT model can only process input tokens up to 512. Following \cite{mao2021dyle}, we group consecutive sentences of a long document into \textit{chunks}. We set the maximum length at 512 and allow for 20\% overlapping with the previous chunk. This way we could include the intermediate sentences in multiple chunks, wishing to capture local dependencies within the same section or paragraph. We additionally employ the similar greedy algorithm in EXT\_ORACLE to construct the extractive labels for model training. Due to the limitation of computing resources, we set the maximum input length as 1,024 and 6,144 for BART-large and LED model respectively. For neural based models, we finetune models for at most 5 epochs with a learning rate of 2e-5, batch size of 1 with gradient accumulation steps at 4. We save the checkpoints at every 1,000 steps, utilizing early stopping based on ROUGE-2 F1 scores and report the average of 3 best checkpoints on validation set. 

\subsection{Evaluation Metrics}
For automatic evaluation, we report ROUGE-1, ROUGE-2, and ROUGE-LSum. We additionally report BERTScore \cite{bert-score} to measure the semantic meanings of the generated summary. 
\section{Results and Analysis}\label{sec:result}
We discuss the evaluation results and effects in this section and aim to answer multiple research questions.\\
\textbf{RQ1: How well can the extractive methods perform while comparing against the human-written summaries}
Table \ref{tab:all_result} shows the evaluation results on the test set. In row 1 and 2, IRC\_ORACLE can be viewed as an upper-bound for an extractive model that could accurately capture all ``Issue Reason Conclusion'' sentences in the original article. The high rouge scores imply that there exist a substantial amount of content overlapping when legal experts draft the abstractive summary, and thus extractive methods could produce high-quality candidates. \\
\textbf{RQ2: How do the unsupervised and supervised baselines work on the legal texts}
row 3-8 demonstrate the performances of frequently used unsupervised baselines. We observe that the performances are not as good as the supervised abstractive methods (row 12 and 14). Meanwhile, the traditional approaches such as LexRank and TextRank suffer from the redundant contents selection (700 tokens v.s. the reference's 240 tokens in selected sentences).\\
\textbf{RQ3: would the incorporation of longer input bring benefits for supervised extractive summarziation?}
Since there are overlapping between different chunks of the test file, we propose a simple method to post-processing all extracted sentences from the same article but within different chunks and name it as BERT\textsubscript{EXT} - selection. (We group all sentences together, de-duplicate and sort the sentences based on their original order in the article). This brings over 20 ROUGE-1 improvements, 8.7 ROUGE-2 improvements, and 18.77 ROUGE-LSum improvements comparing to the baseline model which is only exposed to the first 512 tokens. This suggests that the truncation of texts would result in the loss of information. \\
\textbf{RQ4: Whether the proposed structure-based generation lead to better performance?} We mainly compare the model's performance on the abstractive summarization in row 12-15. We observe stable improvements across all three ROUGE scores and minor improvements on BertScore. This suggests that the summaries generated by our approach is closer to the oracle references, thus being more readable and understandable. \\
Meanwhile, to 

\textbf{RQ5: Would more training data help?} The original CANLLI dataset comes with around 28k case and summary pairs. To validate this hypothesis, we retrain two baseline models of BART and LED on the non-overlapped 27k pairs that are not annotated with IRC, and report the model's performance in row 16 and 17. Not surprisingly, around 5 points improvements in all ROUGE scores are obtained, suggesting that the larger training data could benefit the model's capbilty to better summarize the salient information in long legal case documents.
\begin{table*}[h!]
\small
% \scriptsize 
    \centering
    % \setlength\tabcolsep{2.1pt}
    \renewcommand{\arraystretch}{1.1}%Tighter
    \begin{tabular}{c|l|ccc|ccc|c}
    %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
    \toprule
    ID &  & \multicolumn{3}{c}{\textbf{Quality}} & \multicolumn{3}{|c}{\textbf{BertScore}} &\multicolumn{1}{|c}{\textbf{Length Metrics}} \\
    
      &   &   R-1 & R-2 & R-L  & F1 &  P  &  R & Abs. Len \\
         \midrule
         & Reference &  -- &	 -- &	 --  & -- & -- & -- & 240.31  \\
         
         \midrule
         \multicolumn{9}{c}{\textbf{Extractive Methods}} \\
         \midrule
         1 & IRC\_ORACLE & 57.92 & 35.72 & 55.05 &88.15& 87.78& 88.57 & 243.09 \\
        2 &  EXT ORACLE (R-L, F1) & 61.41 & 40.44 & 59.08 & 88.19& 87.51& 88.97 & 209.37 \\
         \midrule 
         
           \multicolumn{9}{l}{\textit{unsupervised}} \\
           3 & LSA \cite{Steinberger2004UsingLS} & 38.15 & 18.22 & 35.76 & 84.63& 83.48& 85.84 & 787.98  \\
           4 & LexRank \cite{erkan2004lexrank} & 38.63 & 17.70 & 35.87 & 84.40& 83.47& 85.39 & 705.56 \\
            5 & TextRank \cite{DBLP:journals/corr/BarriosLAW16}  & 36.70 & 16.19 & 34.00 & 83.53& 82.20& 84.95 & 722.46  \\
            6 & PACSUM \cite{zheng-lapata-2019-sentence} & 39.24 & 14.31 & 36.80 & 81.64& 79.80& 83.60 & 188.44\\
           7 & PACSUM - LEGAL\_BERT & 37.83 & 13.50 & 35.42  &   81.54& 79.67& 83.53& 188.21 \\
           8 & HipoRank \cite{dong-etal-2021-discourse} & 42.85 & 17.75&  40.08 & 83.53& 82.10& 85.05 & 228.09 \\
           \midrule
        %   \multicolumn{9}{l}{\textit{supervised}} \\
        %   BERT\textsubscript{EXT} - selection & -- & -- & -- \\
           
        %  \midrule
             \multicolumn{9}{l}{\textit{w/o fine-tuning}} \\
        9 &  BERT\textsubscript{EXT} - first 512 token & 18.32 & 7.31& 16.76 &81.77& 82.88& 80.75 & 43.41  \\
      
         10 & BERT\textsubscript{EXT} - selection & 39.14 & 16.38 & 36.40 & 83.84& 82.71& 85.04 & 581.45 \\
          
         \midrule
          \multicolumn{9}{l}{\textit{w/ fine-tuning}} \\

          11 & BERT\textsubscript{EXT} - selection (ckpt 30000) & 40.78 & 17.63 & 37.75 & 84.05& 83.00& 85.19 & 588.60\\
          \midrule
         \multicolumn{9}{c}{\textbf{Abstractive Methods}} \\
         \midrule
       12 & LED   & 49.56 & 23.78 & 46.48  & 86.75& 87.00& 86.56 & 199.47  \\
      
       13 & LED + prompt &  50.69	& 24.33	& 47.53 & 86.87& 86.84& 86.95 & 223.58  \\
       14 &  BART  & 47.93 & 22.34 & 44.74 &  86.16& 85.59& 86.81 & 284.08 \\
        15& BART  + prompt & 51.44 & 23.29 & 47.99  &86.51& 86.12& 86.95 & 250.40 \\
       
       \midrule 
       \multicolumn{9}{l}{\textit{w/ larger training data}}\\
       16 &  BART + larger train & 50.47 & 25.15 & 46.60 & 87.27& 87.77& 86.82 & 172.86\\
       17 &  LED + larger train & 54.41 &  29.57 & 51.17 & 87.86& 87.82& 87.95 & 234.16 \\
       

        % \midrule
        % \multicolumn{9}{l}{\textit{Different Styles}} \\
        %  Style-1 &  48.33 &	22.88 &	45.05 & 0.9613  &  9.16  &  0.74 & 210.60 & 0.1183 \\
        %  Style-2 &  48.28 &	22.61 &	44.99 & 0.9623  &  9.16  &  0.74 & 214.57 & 0.1192 \\
        %  Style-3 &  41.89 &	18.83 &	39.16 & 0.9621  &  8.29  &  0.73 & 142.75 & 0.0808 \\
        % Style-4 &  48.61 &	\textbf{23.24} &	{45.61} & 0.9627  &  9.56  &  0.74 & 223.58 & 0.1212 \\
           
        % \midrule
        
        \bottomrule
        
    \end{tabular}
    \caption{Model Performance for the original test set with 106 instances from the 1049 annotated dataset.}
    \label{tab:all_result}
\end{table*}

% OLD TABLE with abstractedness and density. 
% \begin{table*}[t!]
% \small
% % \scriptsize 
%     \centering
%     % \setlength\tabcolsep{2.1pt}
%     \renewcommand{\arraystretch}{1.1}%Tighter
%     \begin{tabular}{l|ccc|ccc|cc}
%     %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
%     \toprule
%     & \multicolumn{3}{c}{\textbf{Quality}} & \multicolumn{3}{|c}{\textbf{Abstractiveness}} &\multicolumn{2}{|c}{\textbf{Length Metrics}} \\
    
%          &   R-1& R-2 & R-L  & Coverage  &  Density  &  2G-overlap & Abs. Len & Comp. Ratio \\
%          \midrule
%          Reference &  -- &	 -- &	 --  & 0.9338  &  7.50  &  0.61 & 240.31 & 0.1242 \\
         
%          \midrule
%          \multicolumn{9}{l}{\textbf{Extractive Methods}} \\
%          IRC\_ORACLE & 57.92 & 35.72 & 55.05 & 0.6559 & 2.18 & 0.18 & 243.09 & 0.1511\\
%          EXT ORACLE & 61.41 & 40.44 & 59.08 \\
%          \midrule 
%              \multicolumn{9}{l}{\textit{w/o fine-tuning}} \\
%          BERT\textsubscript{EXT} - first 512 token & 18.32 & 7.31& 16.76 & 0.6184 & 2.05 & 0.20 & 43.41 & 0.0260 \\
      
%           BERT\textsubscript{EXT} - selection & 39.14 & 16.38 & 36.40 & 0.6340 & 2.19 & 0.16 & 581.45 & 0.3674\\
%           \midrule
%           \multicolumn{9}{l}{\textit{unsupervised methods}} \\
%             TEXTRANK \cite{DBLP:journals/corr/BarriosLAW16}  & 32.82 & 16.37 & 30.81 \\
%             PACSUM \cite{zheng-lapata-2019-sentence} & 38.10 & 14.14 & 35.82 \\
%             PACSUM - LegalBert & 37.60 & 13.58 & 35.22 \\
%           \midrule
%           \multicolumn{9}{l}{\textit{supervised}} \\
%           BERT\textsubscript{EXT} - selection & -- & -- & -- \\
           
%          \midrule
%          \midrule
%          \multicolumn{9}{l}{\textbf{Abstractive Methods}} \\
%       LED  -- no prompt & 49.56 & 23.78 & 46.48  & 0.9655  &  10.61  &  0.77 & 199.47 & 0.1097 \\
%         LED &  50.69	& 24.33	& 47.53 & 0.9627  &  9.56  &  0.74 & 223.58 & 0.1212 \\
%         BART -- no prompt & 47.93 & 22.34 & 44.74 &  0.9508 & 8.83 & 0.68 & 284.08 & 0.1609\\
%         BART  & 51.44 & 23.29 & 47.99  & 0.9507 &  8.49  &  0.68 & 250.40 & 0.1402 \\
        
%         \midrule
%         \multicolumn{9}{l}{\textit{Different Styles}} \\
%          Style-1 &  48.33 &	22.88 &	45.05 & 0.9613  &  9.16  &  0.74 & 210.60 & 0.1183 \\
%          Style-2 &  48.28 &	22.61 &	44.99 & 0.9623  &  9.16  &  0.74 & 214.57 & 0.1192 \\
%          Style-3 &  41.89 &	18.83 &	39.16 & 0.9621  &  8.29  &  0.73 & 142.75 & 0.0808 \\
%         Style-4 &  48.61 &	\textbf{23.24} &	{45.61} & 0.9627  &  9.56  &  0.74 & 223.58 & 0.1212 \\
           
%         % \midrule
        
%         \bottomrule
        
%     \end{tabular}
%     \caption{Model Performance}
%     \label{tab:all_result}
% \end{table*}


% \begin{table*}[t!]
% \small
% % \scriptsize 
%     \centering
%     % \setlength\tabcolsep{2.1pt}
%     \renewcommand{\arraystretch}{1.1}%Tighter
%     \begin{tabular}{l|ccc|ccc|cc}
%     %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
%     \toprule
%     & \multicolumn{3}{c}{\textbf{Quality}} & \multicolumn{3}{|c}{\textbf{BertScore}} &\multicolumn{2}{|c}{\textbf{Length Metrics}} \\
    
%          &   R-1 & R-2 & R-L  & P  &  R  &  F1 & Abs. Len & Comp. Ratio \\
%          \midrule
%          Reference &  -- &	 -- &	 --  & 0.9338  &  7.50  &  0.61 & 240.31 & 0.1242 \\
         
%          \midrule
%          \multicolumn{9}{c}{\textbf{Extractive Methods}} \\
%          \midrule
%          IRC\_ORACLE &  -- & -- & -- & \\
%          EXT ORACLE (R-L, F1) &  -- & -- & -- & \\
%          \midrule 
         
%           \multicolumn{9}{l}{\textit{unsupervised methods}} \\
%           LSA \cite{Steinberger2004UsingLS} & -- & -- & -- \\
%           LexRank \cite{erkan2004lexrank}  & -- & -- & -- \\
%             TextRank \cite{DBLP:journals/corr/BarriosLAW16}  & -- & -- & -- \\
%             PACSUM \cite{zheng-lapata-2019-sentence}  & -- & -- & -- \\
            
%             HipoRank \cite{dong-etal-2021-discourse} &  & -- & -- & --\\
%           \midrule
%         %   \multicolumn{9}{l}{\textit{supervised}} \\
%         %   BERT\textsubscript{EXT} - selection & -- & -- & -- \\
           
%         %  \midrule
%              \multicolumn{9}{l}{\textit{w/o fine-tuning}} \\
%           BERT\textsubscript{EXT} - selection & 39.14 & 16.38 & 36.40 & 0.6340 & 2.19 & 0.16 & 581.45 & 0.3674\\
          
%          \midrule
%          \multicolumn{9}{c}{\textbf{Abstractive Methods}} \\
%          \midrule
%       LED  -- no prompt &  53.72 & 28.75 & 50.17 & 87.55& 87.38& 87.77   \\
%         BART -- no prompt & 50.50 & 25.58 & 46.82 & 87.25& 87.71& 86.84 \\
        
%         \bottomrule
        
%     \end{tabular}
%     \caption{Model Performance trained on 27241 pairs and evaluated on all 1049 annotated sentences.}
%     \label{tab:all_result}
% \end{table*}


==> arxived/Controlled_Generation_Experiment_Setup.tex <==
\section{Controllable Summary Generation}
We frame the controllable summary generation as a natural language generation task. We compare our proposed approach with multiple baselines for both extractive and abstractive summarization in \S \ref{sec:result} using multiple automatic metrics. We find that the structure aware summary generation outperforms vanilla models. We additionally propose a salient rewarding metrics that can more precisely evaluate the coverage and adherence of generation result while giving the user provided prompt.

\subsection{Structure Guided Summary Generation}
From the corpus released by (cite Huihui's newest paper),  annotators are asked to annotate individual sentences in the summary following the IRC schema (described in \S dataset). Thus, the annotated data comes with a label sequence which represents the structure of the summary. One example can be found in Figure \ref{}. For the abstractive summarziation models, we add the annotated text sequence before the original texts, thus letting the model to implicitly map the structure sequence to the generation summary sentences.

% \subsection{Long Input Split}
% Most neural extrative summarizers are limited by the length of inputs, which is usually 512 tokens cite{BERT} and fall far below the average length of 5k tokens in the legal documents. It is impractical to concatenate all sentences in a document and encode them with a large pretrained model. Following \cite{mao2021dyle}, we group consecutive sentences into \textit{chunks}. We set the maximum length at 512 and allow for 20\% overlapping with the previous chunk. This way we could include the intermediate sentences in multiple chunks, wishing to capture local dependencies within the same section or paragraph. 

\subsection{Extractive Summarization}
\paragraph{Extractive oracles.} \textit{Extractive oracles} denotes a set of selected text snippets whose concatenation maximizes the evaluation metric given the gold summary. We first utilize the \textbf{IRC\_Oracle}, which sentences manually labelled with the IRC types are concatenated together to form a extractive summary. Following \cite{nallapati2017summarunner}, we additionally report \textbf{EXT\_ORACLE}, a baseline for an
oracle summarizer \cite{nallapati2017summarunner}, which greedily select sentences from the original article based on the ROUGE-L scores comparing to the abstractive summary.

\paragraph{Extractive Baselines}
We compare the proposed framework with various baselines. For unsupervised extractive summarization models, we compare with LSA  \cite{Steinberger2004UsingLS},
LexRank \cite{erkan2004lexrank}, TextRank \cite{DBLP:journals/corr/BarriosLAW16}, PACSUM \cite{zheng-lapata-2019-sentence}. We further include HipoRank \cite{dong-etal-2021-discourse}, which achieved the state of the art performance on scientific paper summarization, which also has long text inputs.
For supervised methods, BERTEXT \cite{liu-lapata-2019-text} uses a novel document-level encoder based on BERT which is able to express the semantics of a document and obtain representations for
its sentences. 

\subsection{Abstractive Summarization}
For abstracive summarization, we experiment with BART \cite{lewis-etal-2020-bart} and the Longformer-Encoder-Decoder (LED) \cite{Beltagy2020Longformer}. The latter model can process longer input document up-to 16k tokens. 

\subsection{Implementation Details}
For PACUSUM, we used the released bert checkpoint\footnote{\url{https://github.com/mswellhao/PacSum}}.For BERTEXT without fine-tuning, we use the released checkpoint\footnote{https://github.com/nlpyang/PreSumm} trained on CNN$/$DailyMail Dataset and inference the extracted sentence from each chunk. One limitation of training the BERTEXT model is that the BERT model can only process input tokens up to 512. Following \cite{mao2021dyle}, we group consecutive sentences of a long document into \textit{chunks}. We set the maximum length at 512 and allow for 20\% overlapping with the previous chunk. This way we could include the intermediate sentences in multiple chunks, wishing to capture local dependencies within the same section or paragraph. We additionally employ the similar greedy algorithm in EXT\_ORACLE to construct the extractive labels for model training. Due to the limitation of computing resources, we set the maximum input length as 1,024 and 6,144 for BART-large and LED model respectively. For neural based models, we finetune models for at most 5 epochs with a learning rate of 2e-5, batch size of 1 with gradient accumulation steps at 4. We save the checkpoints at every 1,000 steps, utilizing early stopping based on ROUGE-2 F1 scores and report the average of 3 best checkpoints on validation set. 

\subsection{Evaluation Metrics}
For automatic evaluation, we report ROUGE-1, ROUGE-2, and ROUGE-LSum. We additionally report BERTScore \cite{bert-score} to measure the semantic meanings of the generated summary. 
\section{Results and Analysis}\label{sec:result}
We discuss the evaluation results and effects in this section and aim to answer multiple research questions.\\
\textbf{RQ1: How well can the extractive methods perform while comparing against the human-written summaries}
Table \ref{tab:all_result} shows the evaluation results on the test set. In row 1 and 2, IRC\_ORACLE can be viewed as an upper-bound for an extractive model that could accurately capture all ``Issue Reason Conclusion'' sentences in the original article. The high rouge scores imply that there exist a substantial amount of content overlapping when legal experts draft the abstractive summary, and thus extractive methods could produce high-quality candidates. \\
\textbf{RQ2: How do the unsupervised and supervised baselines work on the legal texts}
row 3-8 demonstrate the performances of frequently used unsupervised baselines. We observe that the performances are not as good as the supervised abstractive methods (row 12 and 14). Meanwhile, the traditional approaches such as LexRank and TextRank suffer from the redundant contents selection (700 tokens v.s. the reference's 240 tokens in selected sentences).\\
\textbf{RQ3: would the incorporation of longer input bring benefits for supervised extractive summarziation?}
Since there are overlapping between different chunks of the test file, we propose a simple method to post-processing all extracted sentences from the same article but within different chunks and name it as BERT\textsubscript{EXT} - selection. (We group all sentences together, de-duplicate and sort the sentences based on their original order in the article). This brings over 20 ROUGE-1 improvements, 8.7 ROUGE-2 improvements, and 18.77 ROUGE-LSum improvements comparing to the baseline model which is only exposed to the first 512 tokens. This suggests that the truncation of texts would result in the loss of information. \\
\textbf{RQ4: Whether the proposed structure-based generation lead to better performance?} We mainly compare the model's performance on the abstractive summarization in row 12-15. We observe stable improvements across all three ROUGE scores and minor improvements on BertScore. This suggests that the summaries generated by our approach is closer to the oracle references, thus being more readable and understandable. \\
Meanwhile, to 

\textbf{RQ5: Would more training data help?} The original CANLLI dataset comes with around 28k case and summary pairs. To validate this hypothesis, we retrain two baseline models of BART and LED on the non-overlapped 27k pairs that are not annotated with IRC, and report the model's performance in row 16 and 17. Not surprisingly, around 5 points improvements in all ROUGE scores are obtained, suggesting that the larger training data could benefit the model's capbilty to better summarize the salient information in long legal case documents.
\begin{table*}[h!]
\small
% \scriptsize 
    \centering
    % \setlength\tabcolsep{2.1pt}
    \renewcommand{\arraystretch}{1.1}%Tighter
    \begin{tabular}{c|l|ccc|ccc|c}
    %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
    \toprule
    ID &  & \multicolumn{3}{c}{\textbf{Quality}} & \multicolumn{3}{|c}{\textbf{BertScore}} &\multicolumn{1}{|c}{\textbf{Length Metrics}} \\
    
      &   &   R-1 & R-2 & R-L  & F1 &  P  &  R & Abs. Len \\
         \midrule
         & Reference &  -- &	 -- &	 --  & -- & -- & -- & 240.31  \\
         
         \midrule
         \multicolumn{9}{c}{\textbf{Extractive Methods}} \\
         \midrule
         1 & IRC\_ORACLE & 57.92 & 35.72 & 55.05 &88.15& 87.78& 88.57 & 243.09 \\
        2 &  EXT ORACLE (R-L, F1) & 61.41 & 40.44 & 59.08 & 88.19& 87.51& 88.97 & 209.37 \\
         \midrule 
         
           \multicolumn{9}{l}{\textit{unsupervised}} \\
           3 & LSA \cite{Steinberger2004UsingLS} & 38.15 & 18.22 & 35.76 & 84.63& 83.48& 85.84 & 787.98  \\
           4 & LexRank \cite{erkan2004lexrank} & 38.63 & 17.70 & 35.87 & 84.40& 83.47& 85.39 & 705.56 \\
            5 & TextRank \cite{DBLP:journals/corr/BarriosLAW16}  & 36.70 & 16.19 & 34.00 & 83.53& 82.20& 84.95 & 722.46  \\
            6 & PACSUM \cite{zheng-lapata-2019-sentence} & 39.24 & 14.31 & 36.80 & 81.64& 79.80& 83.60 & 188.44\\
           7 & PACSUM - LEGAL\_BERT & 37.83 & 13.50 & 35.42  &   81.54& 79.67& 83.53& 188.21 \\
           8 & HipoRank \cite{dong-etal-2021-discourse} & 42.85 & 17.75&  40.08 & 83.53& 82.10& 85.05 & 228.09 \\
           \midrule
        %   \multicolumn{9}{l}{\textit{supervised}} \\
        %   BERT\textsubscript{EXT} - selection & -- & -- & -- \\
           
        %  \midrule
             \multicolumn{9}{l}{\textit{w/o fine-tuning}} \\
        9 &  BERT\textsubscript{EXT} - first 512 token & 18.32 & 7.31& 16.76 &81.77& 82.88& 80.75 & 43.41  \\
      
         10 & BERT\textsubscript{EXT} - selection & 39.14 & 16.38 & 36.40 & 83.84& 82.71& 85.04 & 581.45 \\
          
         \midrule
          \multicolumn{9}{l}{\textit{w/ fine-tuning}} \\

          11 & BERT\textsubscript{EXT} - selection (ckpt 30000) & 40.78 & 17.63 & 37.75 & 84.05& 83.00& 85.19 & 588.60\\
          \midrule
         \multicolumn{9}{c}{\textbf{Abstractive Methods}} \\
         \midrule
       12 & LED   & 49.56 & 23.78 & 46.48  & 86.75& 87.00& 86.56 & 199.47  \\
      
       13 & LED + prompt &  50.69	& 24.33	& 47.53 & 86.87& 86.84& 86.95 & 223.58  \\
       14 &  BART  & 47.93 & 22.34 & 44.74 &  86.16& 85.59& 86.81 & 284.08 \\
        15& BART  + prompt & 51.44 & 23.29 & 47.99  &86.51& 86.12& 86.95 & 250.40 \\
       
       \midrule 
       \multicolumn{9}{l}{\textit{w/ larger training data}}\\
       16 &  BART + larger train & 50.47 & 25.15 & 46.60 & 87.27& 87.77& 86.82 & 172.86\\
       17 &  LED + larger train & 54.41 &  29.57 & 51.17 & 87.86& 87.82& 87.95 & 234.16 \\
       

        % \midrule
        % \multicolumn{9}{l}{\textit{Different Styles}} \\
        %  Style-1 &  48.33 &	22.88 &	45.05 & 0.9613  &  9.16  &  0.74 & 210.60 & 0.1183 \\
        %  Style-2 &  48.28 &	22.61 &	44.99 & 0.9623  &  9.16  &  0.74 & 214.57 & 0.1192 \\
        %  Style-3 &  41.89 &	18.83 &	39.16 & 0.9621  &  8.29  &  0.73 & 142.75 & 0.0808 \\
        % Style-4 &  48.61 &	\textbf{23.24} &	{45.61} & 0.9627  &  9.56  &  0.74 & 223.58 & 0.1212 \\
           
        % \midrule
        
        \bottomrule
        
    \end{tabular}
    \caption{Model Performance for the original test set with 106 instances from the 1049 annotated dataset.}
    \label{tab:all_result}
\end{table*}

% OLD TABLE with abstractedness and density. 
% \begin{table*}[t!]
% \small
% % \scriptsize 
%     \centering
%     % \setlength\tabcolsep{2.1pt}
%     \renewcommand{\arraystretch}{1.1}%Tighter
%     \begin{tabular}{l|ccc|ccc|cc}
%     %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
%     \toprule
%     & \multicolumn{3}{c}{\textbf{Quality}} & \multicolumn{3}{|c}{\textbf{Abstractiveness}} &\multicolumn{2}{|c}{\textbf{Length Metrics}} \\
    
%          &   R-1& R-2 & R-L  & Coverage  &  Density  &  2G-overlap & Abs. Len & Comp. Ratio \\
%          \midrule
%          Reference &  -- &	 -- &	 --  & 0.9338  &  7.50  &  0.61 & 240.31 & 0.1242 \\
         
%          \midrule
%          \multicolumn{9}{l}{\textbf{Extractive Methods}} \\
%          IRC\_ORACLE & 57.92 & 35.72 & 55.05 & 0.6559 & 2.18 & 0.18 & 243.09 & 0.1511\\
%          EXT ORACLE & 61.41 & 40.44 & 59.08 \\
%          \midrule 
%              \multicolumn{9}{l}{\textit{w/o fine-tuning}} \\
%          BERT\textsubscript{EXT} - first 512 token & 18.32 & 7.31& 16.76 & 0.6184 & 2.05 & 0.20 & 43.41 & 0.0260 \\
      
%           BERT\textsubscript{EXT} - selection & 39.14 & 16.38 & 36.40 & 0.6340 & 2.19 & 0.16 & 581.45 & 0.3674\\
%           \midrule
%           \multicolumn{9}{l}{\textit{unsupervised methods}} \\
%             TEXTRANK \cite{DBLP:journals/corr/BarriosLAW16}  & 32.82 & 16.37 & 30.81 \\
%             PACSUM \cite{zheng-lapata-2019-sentence} & 38.10 & 14.14 & 35.82 \\
%             PACSUM - LegalBert & 37.60 & 13.58 & 35.22 \\
%           \midrule
%           \multicolumn{9}{l}{\textit{supervised}} \\
%           BERT\textsubscript{EXT} - selection & -- & -- & -- \\
           
%          \midrule
%          \midrule
%          \multicolumn{9}{l}{\textbf{Abstractive Methods}} \\
%       LED  -- no prompt & 49.56 & 23.78 & 46.48  & 0.9655  &  10.61  &  0.77 & 199.47 & 0.1097 \\
%         LED &  50.69	& 24.33	& 47.53 & 0.9627  &  9.56  &  0.74 & 223.58 & 0.1212 \\
%         BART -- no prompt & 47.93 & 22.34 & 44.74 &  0.9508 & 8.83 & 0.68 & 284.08 & 0.1609\\
%         BART  & 51.44 & 23.29 & 47.99  & 0.9507 &  8.49  &  0.68 & 250.40 & 0.1402 \\
        
%         \midrule
%         \multicolumn{9}{l}{\textit{Different Styles}} \\
%          Style-1 &  48.33 &	22.88 &	45.05 & 0.9613  &  9.16  &  0.74 & 210.60 & 0.1183 \\
%          Style-2 &  48.28 &	22.61 &	44.99 & 0.9623  &  9.16  &  0.74 & 214.57 & 0.1192 \\
%          Style-3 &  41.89 &	18.83 &	39.16 & 0.9621  &  8.29  &  0.73 & 142.75 & 0.0808 \\
%         Style-4 &  48.61 &	\textbf{23.24} &	{45.61} & 0.9627  &  9.56  &  0.74 & 223.58 & 0.1212 \\
           
%         % \midrule
        
%         \bottomrule
        
%     \end{tabular}
%     \caption{Model Performance}
%     \label{tab:all_result}
% \end{table*}


% \begin{table*}[t!]
% \small
% % \scriptsize 
%     \centering
%     % \setlength\tabcolsep{2.1pt}
%     \renewcommand{\arraystretch}{1.1}%Tighter
%     \begin{tabular}{l|ccc|ccc|cc}
%     %\begin{tabular}{l|lllc|lllc|p{0.9cm}ll}
%     \toprule
%     & \multicolumn{3}{c}{\textbf{Quality}} & \multicolumn{3}{|c}{\textbf{BertScore}} &\multicolumn{2}{|c}{\textbf{Length Metrics}} \\
    
%          &   R-1 & R-2 & R-L  & P  &  R  &  F1 & Abs. Len & Comp. Ratio \\
%          \midrule
%          Reference &  -- &	 -- &	 --  & 0.9338  &  7.50  &  0.61 & 240.31 & 0.1242 \\
         
%          \midrule
%          \multicolumn{9}{c}{\textbf{Extractive Methods}} \\
%          \midrule
%          IRC\_ORACLE &  -- & -- & -- & \\
%          EXT ORACLE (R-L, F1) &  -- & -- & -- & \\
%          \midrule 
         
%           \multicolumn{9}{l}{\textit{unsupervised methods}} \\
%           LSA \cite{Steinberger2004UsingLS} & -- & -- & -- \\
%           LexRank \cite{erkan2004lexrank}  & -- & -- & -- \\
%             TextRank \cite{DBLP:journals/corr/BarriosLAW16}  & -- & -- & -- \\
%             PACSUM \cite{zheng-lapata-2019-sentence}  & -- & -- & -- \\
            
%             HipoRank \cite{dong-etal-2021-discourse} &  & -- & -- & --\\
%           \midrule
%         %   \multicolumn{9}{l}{\textit{supervised}} \\
%         %   BERT\textsubscript{EXT} - selection & -- & -- & -- \\
           
%         %  \midrule
%              \multicolumn{9}{l}{\textit{w/o fine-tuning}} \\
%           BERT\textsubscript{EXT} - selection & 39.14 & 16.38 & 36.40 & 0.6340 & 2.19 & 0.16 & 581.45 & 0.3674\\
          
%          \midrule
%          \multicolumn{9}{c}{\textbf{Abstractive Methods}} \\
%          \midrule
%       LED  -- no prompt &  53.72 & 28.75 & 50.17 & 87.55& 87.38& 87.77   \\
%         BART -- no prompt & 50.50 & 25.58 & 46.82 & 87.25& 87.71& 86.84 \\
        
%         \bottomrule
        
%     \end{tabular}
%     \caption{Model Performance trained on 27241 pairs and evaluated on all 1049 annotated sentences.}
%     \label{tab:all_result}
% \end{table*}

